Global News Synchrony and Diversity During the Start of the COVID-19 Pandemic

News coverage profoundly affects how countries and individuals behave in international relations. Yet, we have little empirical evidence of how news coverage varies across countries. To enable studies of global news coverage, we develop an efficient computational methodology that comprises three components: (i) a transformer model to estimate multilingual news similarity; (ii) a global event identification system that clusters news based on a similarity network of news articles; and (iii) measures of news synchrony across countries and news diversity within a country, based on country-specific distributions of news coverage of the global events. Each component achieves state-of-the art performance, scaling seamlessly to massive datasets of millions of news articles. We apply the methodology to 60 million news articles published globally between January 1 and June 30, 2020, across 124 countries and 10 languages, detecting 4357 news events. We identify the factors explaining diversity and synchrony of news coverage across countries. Our study reveals that news media tend to cover a more diverse set of events in countries with larger Internet penetration, more official languages, larger religious diversity, higher economic inequality, and larger populations. Coverage of news events is more synchronized between countries that not only actively participate in commercial and political relations -- such as, pairs of countries with high bilateral trade volume, and countries that belong to the NATO military alliance or BRICS group of major emerging economies -- but also countries that share certain traits: an official language, high GDP, and high democracy indices.

==> tables/pub_agreements.tex <==

% Source: https://vw-project.slack.com/archives/C01EJ90U4NQ/p1629312987302600?thread_ts=1629225069.287500&cid=C01EJ90U4NQ
% We need to recompute these numbers using Fabian's script:
% without Chengzhi and Po-Tsun:
% [1] "GEO"
% [1] ":::"
% [1] "GWET:"
% [1] 0.74687
% [1] "Krippendorff:"
% [1] 0.74662
% [1] "-------------------------------------------"
% [1] "ENT"
% [1] ":::"
% [1] "GWET:"
% [1] 0.8298
% [1] "Krippendorff:"
% [1] 0.75577
% [1] "-------------------------------------------"
% [1] "TIME"
% [1] ":::"
% [1] "GWET:"
% [1] 0.77417
% [1] "Krippendorff:"
% [1] 0.38592
% [1] "-------------------------------------------"
% [1] "NAR"
% [1] ":::"
% [1] "GWET:"
% [1] 0.74003
% [1] "Krippendorff:"
% [1] 0.66973
% [1] "-------------------------------------------"
% [1] "OVERALL"
% [1] ":::"
% [1] "GWET:"
% [1] 0.82172
% [1] "Krippendorff:"
% [1] 0.77978
% [1] "-------------------------------------------"
% [1] "TONE"
% [1] ":::"
% [1] "GWET:"
% [1] 0.57229
% [1] "Krippendorff:"
% [1] 0.51547
% [1] "-------------------------------------------"
% [1] "STYLE"
% [1] ":::"
% [1] "GWET:"
% [1] 0.55027
% [1] "Krippendorff:"
% [1] 0.37775
% [1] "-------------------------------------------"


\begin{table}[tb]
    \centering

    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{lrrrrrrr}
    \toprule
     &  GEO &  ENT & TIME  & NAR & OVERALL  \\
    \midrule
Krippen. & 0.73 & 0.69 & 0.57 & 0.69 & 0.77  \\
Gwet & 0.81 & 0.67 & 0.75 & 0.69 & 0.76  \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Inter-rater agreement measures, Krippendorf's $\alpha$ and Gwet's AC$_{1}$, for each labeled dimension.}
    \label{tab:agreements}
\end{table}


==> tables/pub_annotators_pearson_with_mean.tex <==
\begin{table}[tbh]
    \centering

    \scalebox{0.84}{
    \begin{tabular}{lrrrrr}
    \toprule
    id &  items &  shared & seconds/item  &  correlation \\
    \midrule
    1  &    1,657 &            809 &            296 &     0.88 \\
    2  &    2,311 &            495 &            344 &     0.86 \\
    3  &    1,197 &            611 &            237 &     0.85 \\
    4  &    1,178 &            794 &            213 &     0.85 \\
    5  &     134 &             98 &            153 &     0.84 \\
    6  &    1,036 &            626 &            128 &     0.84 \\
    7  &    1,302 &            345 &            220 &     0.84 \\
    8  &     466 &            398 &            224 &     0.84 \\
    9  &     787 &            208 &            233 &     0.84 \\
    10 &     887 &            368 &            506 &     0.83 \\
    11 &    1,062 &            466 &            387 &     0.82 \\
    12 &     361 &            321 &            311 &     0.81 \\
    13 &     262 &            213 &            165 &     0.81 \\
    14 &     139 &            135 &            235 &     0.79 \\
    15 &    1,076 &            716 &             71 &     0.77 \\
    % 1  &    3300 &           1150 &            262 &     0.88 \\
    % 2  &    1522 &           1006 &            196 &     0.85 \\
    % 3  &    4275 &            633 &            260 &     0.85 \\
    % 4  &    1685 &            850 &            227 &     0.85 \\
    % 5  &     529 &            451 &            216 &     0.85 \\
    % 6  &    1200 &            743 &            121 &     0.84 \\
    % 7  &    1803 &            235 &            178 &     0.84 \\
    % 8  &    1762 &            383 &            189 &     0.83 \\
    % 9  &    1286 &            418 &            506 &     0.82 \\
    % 10 &     508 &            442 &            219 &     0.81 \\
    % 11 &     300 &            258 &            158 &     0.80 \\
    % 12 &    2571 &            795 &            272 &     0.80 \\
    % 13 &     148 &            148 &            230 &     0.78 \\
    % 14 &    1589 &           1094 &             66 &     0.78 \\
    % 15 &     198 &            158 &            106 &     0.73 \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{Annotators and their statistics: the number of labeled items (news article pairs), the number of shared items (also annotated by another annotator), median number of seconds to label an item, and Pearson correlation of their OVERALL labels with the mean labels of other annotators. Only annotators with at least 100 labels are shown.}
    \label{tab:annotators}
\end{table}


==> tables/pub_lang1_pearson_with_mean.tex <==
\begin{table}[tb]
    \centering
    
    \scalebox{0.84}{
    \begin{tabular}{lrr}
    \toprule
    languages &  annotations &  mean(OVERALL) \\
    \midrule
       en &    5,189 &         2.92 \\
       de &    2,166 &         2.56 \\
       es &     955 &         2.40 \\
       zh &     866 &         2.24 \\
     de-en &     863 &         3.20 \\
       tr &     817 &         2.79 \\
       pl &     584 &         2.36 \\
       ar &     572 &         2.41 \\
     es-en &     504 &         2.79 \\
       it &     411 &         2.65 \\
     es-it &     320 &         2.29 \\
       ru &     289 &         2.78 \\
     zh-en &     253 &         3.04 \\
       fr &     184 &         2.39 \\
     de-fr &     116 &         1.88 \\
     pl-en &      77 &         2.38 \\
     de-pl &      35 &         1.69 \\
     fr-pl &      11 &         1.91 \\
    %   en &    6,419 &         2.89 \\
    %   de &    3,251 &         2.56 \\
    %   zh &    2,784 &         2.30 \\
    %   es &    2,238 &         2.35 \\
    %  de-en &    1,949 &         2.94 \\
    %   ar &    1,640 &         2.66 \\
    %   tr &    1,238 &         2.63 \\
    %   it &     803 &         2.64 \\
    %  es-en &     759 &         2.84 \\
    %   pl &     741 &         2.35 \\
    %  zh-en &     523 &         2.97 \\
    %  es-it &     474 &         2.29 \\
    %   ru &     350 &         2.77 \\
    %   fr &     267 &         2.15 \\
    %  de-fr &     178 &         1.92 \\
    %  pl-en &     119 &         2.35 \\
    %  fr-en &      99 &         1.22 \\
    %  fr-pl &      53 &         1.67 \\
    %  de-pl &      47 &         1.69 \\
    \bottomrule
    \end{tabular}
    }
    
    \caption{The number of annotations and the mean OVERALL label (the higher, the more dissimilar) across the 10 languages and their combinations.}
    \label{tab:lang_dist}
\end{table}


